Few-shot Image Generation Using Discrete Content Representation

Few-shot image generation and few-shot image translation are two related tasks, both of which aim to generate new images for an unseen category with only a few images. In this work, we make the first attempt to adapt few-shot image translation method to few-shot image generation task. Few-shot image translation disentangles an image into style vector and content map. An unseen style vector can be combined with different seen content maps to produce different images. However, it needs to store seen images to provide content maps and the unseen style vector may be incompatible with seen content maps. To adapt it to few-shot image generation task, we learn a compact dictionary of local content vectors via quantizing continuous content maps into discrete content maps instead of storing seen images. Furthermore, we model the autoregressive distribution of discrete content map conditioned on style vector, which can alleviate the incompatibility between content map and style vector. Qualitative and quantitative results on three real datasets demonstrate that our model can produce images of higher diversity and fidelity for unseen categories than previous methods.

==> Sections/figures/effect_dictionary_length.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=0.24]{./Figures/.png}
\end{center}
\caption{Evaluating the effect of the length of dictionary of local content vectors. From top to bottom: unseen style images, generated .}
\label{fig:dictionary_length} 
\end{figure}

==> Sections/figures/motivation1.tex <==
\begin{figure}
\begin{center}
\includegraphics[scale=1.5]{./Figures/motivation1.png}
\end{center}
\caption{The illustration of extending few-shot image translation method to our few-shot image generation method. For few-shot image translation,  category-invariant content codes are extracted from seen images and stored in repository in the training phase. In the testing phase, content codes are chosen from the repository to combine with style code of unseen image for producing translation images. For our few-shot image generation framework, in the training phase, a content code dictionary is constructed for  supporting stochastic sampling and a style-content compatibility model is learnt for sampling style-compatible content codes. In the testing phase, given style code of unseen image, we can randomly sample style-compatible content codes based on content code dictionary and style-content compatible model to produce diverse and realistic images.} 
\label{fig:motivation} 
\end{figure}


% The illustration of extending few-shot image translation method to our few-shot image generation method. For few-shot image generation framework,  category-invariant content codes are extracted from seen images and stored in repository in the training phase. In the testing phase, style-independent content codes are chosen from content code repository to combine with style code of unseen image for producing translation images. For our few-shot image generation framework, in the training phase, a content code dictionary is constructed for  supporting stochastic sampling and a style-content compatibility model is learnt for sampling style-compatible content codes. In the testing phase, given style code of unseen image, we can randomly sample style-compatible content codes based on content code dictionary and style-content compatible model to produce diverse and realistic images.

==> Sections/figures/storage_comparison.tex <==
%\begin{figure}
%\begin{center}
%\includegraphics[scale=0.5]{./Figures/memory_comparison.png}
%\end{center}
%% \caption{Comparison between few-shot image translation and few-shot image generation. Few shot image translation model aims at translating random seen images to a unseen category conditioned on a unseen images. Our few-shot image generation method targets at sampling style-aware content maps from learned dictionary to generate new images conditioned on a unseen image.} 
%\caption{Storage cost comparison between few-shot image translation methods and our few-shot image generation method. The former stores seen images to provide content maps, while the latter only stores a compact dictionary of local content vectors. }
%\label{fig:storage_curve} 
%\end{figure}
% The illustration of extending few-shot image translation method to our few-shot image generation method. For few-shot image generation framework,  category-invariant content codes are extracted from seen images and stored in repository in the training phase. In the testing phase, style-independent content codes are chosen from content code repository to combine with style code of unseen image for producing translation images. For our few-shot image generation framework, in the training phase, a content code dictionary is constructed for  supporting stochastic sampling and a style-content compatibility model is learnt for sampling style-compatible content codes. In the testing phase, given style code of unseen image, we can randomly sample style-compatible content codes based on content code dictionary and style-content compatible model to produce diverse and realistic images.

==> Sections/figures/visualization_supple_1st_stage.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.51]{./Figures/vis_supple_stage1.png}
\end{center}
\caption{Images generated by FUNIT, COCO-FUNIT, and Disco-FUNIT(1st stage) in 1-shot setting on Flowers, Animal Faces, and NABirds dataset. (from top to bottom: unseen style images, seen content images, images generated by Disco-FUNIT (1st stage)).}
\label{fig:more_images_1stage} 
\end{figure*}

==> Sections/tables/content_encoder.tex <==
\begin{table}[t]
  \caption{The network architecture of our content encoder $E_C$ with quantisation.} 
  \centering
  %\fontsize{8}{8}\selectfont
  \begin{tabular}{cccc}
  \toprule[0.8pt]
     &Layer & Resample  & Output \cr
      
    \hline
     &Image $\bm{x}$  & -    & 128*128*3   \cr
     \hline
     &Conv-64  &  -    &  128*128*64  \cr
     &Conv-128  &   AvgPool   &  64*64*128  \cr
     &Conv-256  &   AvgPool  &  32*32*256  \cr
     &Conv-512  &   AvgPool   &  16*16*512  \cr
      &ResBlk-512  &   -  &  16*16*512  \cr
      &ResBlk-512  &   -  &  16*16*512  \cr
      &Conv-512  &  -    &  16*16*512  \cr
      &Conv-512  &  -    &  16*16*512  \cr
     \hline
  \end{tabular}
%   \vspace{0.1mm}
  \label{tab:content_encoder}
\end{table}

% \begin{table}[t]
%   \caption{The network architecture of our content encoder $E_C$ with quantisation.} 
%   \centering
%   %\fontsize{8}{8}\selectfont
%   \begin{tabular}{ccccc}
%   \toprule[0.8pt]
%   Content Encoder $E_c$
%     \hline
%     $\bm{x} \in  \mathcal{R}^{128*128*3}$ \cr
%      \hline
%     Conv-64 -> $\mathcal{R}^{128*128*64}$  \cr
%      \hline
%      Conv-128 -> $\mathcal{R}^{64*64*128}$  \cr
%      \hline
%      Conv-256 -> $\mathcal{R}^{32*32*256}$  \cr
%      \hline
%      Conv-512 -> $\mathcal{R}^{16*16*512}$  \cr
%      \hline
%     ResBlk-512 -> $\mathcal{R}^{16*16*512}$  \cr
%     \hline
%     ResBlk-512 -> $\mathcal{R}^{16*16*512}$  \cr
%     \hline
%     Conv2D -> $\mathcal{R}^{w*h*d_c}$  \cr
%      \hline
%     Conv2D -> $\mathcal{R}^{w*h*d_c}$  \cr
%   \end{tabular}
% %   \vspace{0.1mm}
%   \label{tab:content_encoder}
% \end{table}

==> Sections/tables/metric_comparison_finetune.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table}[t]
  \caption{FID ($\downarrow$) and LPIPS ($\uparrow$) of images generated by different methods for 10 selected unseen categories on Flowers dataset.} 
  \centering
%   \fontsize{8}{8}\selectfont
  \resizebox{0.9\columnwidth}{!} {
  \begin{tabular}{l|r|r|r}  
    \hline
     Setting&  FID $\downarrow$  & LPIPS $\uparrow$ & Accuracy(\%) $\uparrow$ \cr
    \hline
    Ojha et al. 2021 & & & \cr
    \hline
    Disco-FUNIT & \textbf{} & \textbf{}  & \textbf{}  \cr
    \hline
  \end{tabular}
  }
  \label{tab:comparison_metric_finetune}
\end{table}




==> Sections/tables/model_parameters.tex <==
% \begin{table}[t]
%   \caption{The number of model parameters of MatchingGAN~\cite{hong2020matchinggan}, F2GAN~\cite{hong2020f2gan}, DAWSON~\cite{liang2020dawson}, DAGAN~\cite{antoniou2017data}, DeltaGAN~\cite{hong2020deltagan}, and our method.} 
%   \centering
%   %\fontsize{8}{8}\selectfont
%   \begin{tabular}{l|r|r}  
%     \toprule[0.8pt]
%      Setting& Training phase   & Testing phase \cr
%     \hline
%     MatchingGAN~\cite{hong2020matchinggan} & 30.3M & 9.8M \cr
%     \hline
%     F2GAN~\cite{hong2020f2gan} &31.1M  &9.9M \cr
%     \hline
%     DAWSON~\cite{liang2020dawson} \cr
%     \hline
%     DAGAN~\cite{antoniou2017data} \cr
%     \hline
%     DeltaGAN~\cite{hong2020deltagan} &33.1M &  8.1M \cr
%     \hline
%     Disco-FUNIT \cr
%     \bottomrule[0.8pt]
%   \end{tabular}
% %   \vspace{0.1mm}
%   \label{tab:model_parameters}
% \end{table}
\begin{table}[t]
  \caption{The number of model parameters of MatchingGAN~\cite{hong2020matchinggan}, F2GAN~\cite{hong2020f2gan}, DAWSON~\cite{liang2020dawson}, DAGAN~\cite{antoniou2017data}, DeltaGAN~\cite{hong2020deltagan}, and our method.} 
  \centering
  %\fontsize{8}{8}\selectfont
  \begin{tabular}{l|r|r}  
    \toprule[0.8pt]
     Setting& Training phase   & Testing phase \cr
    \hline
    MatchingGAN & 30.3M & 9.8M \cr
    \hline
    F2GAN &31.1M  &9.9M \cr
    \hline
    DAWSON \cr
    \hline
    DAGAN \cr
    \hline
    DeltaGAN &33.1M &  8.1M \cr
    \hline
    Disco-FUNIT&113 + 153  &18.6 + 153 \cr
    \bottomrule[0.8pt]
  \end{tabular}
%   \vspace{0.1mm}
  \label{tab:model_parameters}
\end{table}

==> Sections/tables/significance_test.tex <==
\begin{table}[t]
  \caption{The results (Mean±Std) of 10 runs for our method and DeltaGAN~\cite{hong2020deltagan} on Animal Faces dataset in $1$-shot setting.} 
  \centering
  %\fontsize{8}{8}\selectfont
  \begin{tabular}{lrrr}  
    \toprule[0.8pt]
     Setting& Accuracy(\%) $\uparrow$  & FID $\downarrow$  & LPIPS $\uparrow$ \cr
    \hline
     DeltaGAN& 89.81±0.33 & 0.4418±0.19 & 60.31±0.22\cr
    \hline
   Disco-FUNIT & $\textbf{71.44±0.21}$ &$\textbf{0.4511±0.09}$  & $\textbf{61.85±0.15}$   \cr
   \hline
  \end{tabular}
%   \vspace{0.1mm}
  \label{tab:significant_test}
\end{table}

==> Sections/tables/test_time.tex <==
%\begin{table}[t]
%  \caption{Spending time of each module in our method. Query denotes the process of looking-up discrete content map from the dictionary of local content vector.} 
%  \centering
%  %\fontsize{8}{8}\selectfont
%  \begin{tabular}{r|r|r|r|r}  
%    \toprule[0.8pt]
%     Modules & $E_s$ & $T_{C|S}$ & Query & F \cr
%    \hline
%    Time(s)&0.0009 & 6.5281 & 0.0016 & 0.0031 \cr
%    \bottomrule[0.8pt]
%  \end{tabular}
%%   \vspace{0.1mm}
%  \label{tab:test_time}
%\end{table}
% funit: style encoder:0.0009, content encoder:0.0021, decoder:0.0031


